Discovery of Rotational Modulations in the Planetary-Mass Companion 2M1207b: Intermediate Rotation Period and Heterogeneous Clouds in a Low Gravity Atmosphere

Rotational modulations of brown dwarfs have recently provided powerful constraints on the properties of ultra-cool atmospheres, including longitudinal and vertical cloud structures and cloud evolution. Furthermore, periodic light curves directly probe the rotational periods of ultra-cool objects. We present here, for the first time, time-resolved high-precision photometric measurements of a planetary-mass companion, 2M1207b. We observed the binary system with HST/WFC3 in two bands and with two spacecraft roll angles. Using point spread function-based photometry, we reach a nearly photon-noise limited accuracy for both the primary and the secondary. While the primary is consistent with a flat light curve, the secondary shows modulations that are clearly detected in the combined light curve as well as in different subsets of the data. The amplitudes are 1.36% in the F125W and 0.78% in the F160W filters, respectively. By fitting sine waves to the light curves, we find a consistent period of $10.7^{+1.2}_{-0.6}$ hours and similar phases in both bands. The J- and H-band amplitude ratio of 2M1207b is very similar to a field brown dwarf that has identical spectral type but different J-H color. Importantly, our study also measures, for the first time, the rotation period for a directly imaged extra-solar planetary-mass companion.

==> tab1.tex <==
\begin{deluxetable}{cccccccc}
\tabletypesize{\scriptsize}
\tablecaption{F125W Photometry Results\label{tab:F125W}}
\tablewidth{0pt}
\tablehead{
\colhead{Orbit} & \colhead{Pos. Angle} & \colhead{Dither} & \colhead{T
- JD$_{0}$} & \colhead{$\mathrm{Flux_{prim}}$} &
\colhead{$\mathrm{Flux_{prim}}$}  &\colhead{$\mathrm{Flux_{comp}}$} & \colhead{$\mathrm{Flux_{comp}}$}\\
  \colhead{}&\colhead{($^{\circ}$)}&\colhead{Position}&\colhead{[hour]}&\colhead{[$\mathrm{e^{-}/s}$]}
  &\colhead{normalized}&\colhead{[$\mathrm{e^{-}/s}$]}&\colhead{normalized}
}

\startdata
       &           &         &       &          &        &        &        \\
       \multirow{11}{*}{1} &  \multirow{11}{*}{202}
                   &       1 & 0.000 & 76400.23 & 0.9842 & 197.47 & 1.0255 \\
      &          &       1 & 0.030 & 77067.92 & 0.9928 & 194.68 & 1.0110 \\
      &          &       1 & 0.059 & 77335.85 & 0.9963 & 194.17 & 1.0084 \\
      &         &       2 & 0.192 & 77461.98 & 0.9907 & 192.72 & 0.9860 \\
      &         &       2 & 0.221 & 77498.89 & 0.9912 & 197.69 & 1.0114 \\
      &         &       2 & 0.251 & 77807.67 & 0.9951 & 194.43 & 0.9947 \\
      &          &       3 & 0.354 & 76836.70 & 0.9896 & 189.01 & 1.0205 \\
      &          &       3 & 0.384 & 77254.05 & 0.9950 & 188.09 & 1.0155 \\
      &          &       3 & 0.413 & 77474.72 & 0.9978 & 184.35 & 0.9953 \\
      &          &       4 & 0.546 & 77188.85 & 0.9915 & 182.92 & 0.9843 \\
      &          &       4 & 0.575 & 77384.02 & 0.9940 & 190.81 &1.0267 \\
      \hline
       &           &         &       &          &        &        &        \\
       \multirow{11}{*}{2} &  \multirow{11}{*}{227}
                 &       1 & 1.594 & 77839.67 & 0.9990 & 194.62 & 1.0401 \\
     &          &       1 & 1.624 & 77952.59 & 1.0005 & 191.95 & 1.0258 \\
     &          &       1 & 1.653 & 77874.77 & 0.9995 & 188.82 & 1.0091 \\
     &          &       2 & 1.786 & 77221.62 & 0.9920 & 192.39 & 0.9974 \\
     &          &       2 & 1.815 & 77989.91 & 1.0019 & 193.38 & 1.0025 \\
     &          &       2 & 1.845 & 77810.97 & 0.9996 & 200.23 & 1.0380 \\
     &          &       3 & 1.948 & 78412.56 & 0.9989 & 199.15 & 1.0223 \\
     &          &       3 & 1.978 & 78506.68 & 1.0001 & 196.32 & 1.0077 \\
     &          &       3 & 2.007 & 78569.23 & 1.0009 & 196.42 & 1.0083 \\
     &          &       4 & 2.139 & 77237.39 & 0.9956 & 202.16 & 1.0228 \\
     &          &       4 & 2.169 & 77530.01 & 0.9994 & 203.36 &
     1.0289 \\
           \hline
       &           &         &       &          &        &        &        \\
       \multirow{12}{*}{3} &  \multirow{12}{*}{202}
                &       1 & 3.188 & 77956.86 & 1.0043 & 191.32 & 0.9936 \\
      &        &       1 & 3.218 & 78179.49 & 1.0072 & 191.70 & 0.9956 \\
      &        &       1 & 3.247 & 78213.98 & 1.0076 & 195.27 & 1.0141 \\
      &        &       2 & 3.379 & 78591.12 & 1.0051 & 203.01 & 1.0386 \\
      &        &       2 & 3.409 & 78608.24 & 1.0054 & 197.20 & 1.0089 \\
      &        &       2 & 3.439 & 78847.12 & 1.0084 & 195.33 & 0.9993 \\
      &        &       3 & 3.542 & 77870.59 & 1.0029 & 184.67 & 0.9971 \\
      &        &       3 & 3.571 & 78204.56 & 1.0072 & 182.92 & 0.9876 \\
      &        &       3 & 3.601 & 78190.32 & 1.0070 & 185.51 & 1.0016 \\
      &        &       4 & 3.733 & 77932.39 & 1.0010 & 187.29 & 1.0078 \\
      &        &       4 & 3.763 & 78139.97 & 1.0037 & 186.62 & 1.0041 \\
      &        &       4 & 3.793 & 78320.57 & 1.0060 & 186.88 & 1.0056
      \\
           \hline
       &           &         &       &          &        &        &        \\
       \multirow{12}{*}{4} &  \multirow{12}{*}{227}
                  &       1 & 4.782 & 77939.05 & 1.0003 & 185.86 & 0.9933 \\
      &          &      1 & 4.811 & 78127.91 & 1.0027 & 189.97 & 1.0153 \\
      &          &       1 & 4.841 & 78240.98 & 1.0042 & 184.40 & 0.9855 \\
      &          &       2 & 4.973 & 77857.88 & 1.0002 & 184.41 & 0.9560 \\
      &          &       2 & 5.003 & 78020.08 & 1.0023 & 190.59 & 0.9880 \\
      &          &       2 & 5.033 & 78140.80 & 1.0038 & 198.42 & 1.0286 \\
      &          &       3 & 5.136 & 78268.69 & 0.9971 & 191.85 & 0.9848 \\
      &          &       3 & 5.165 & 78559.50 & 1.0008 & 195.65 & 1.0043 \\
      &          &       3 & 5.195 & 78640.39 & 1.0018 & 196.62 & 1.0093 \\
      &          &       4 & 5.327 & 77340.36 & 0.9969 & 198.37 & 1.0037 \\
      &          &       4 & 5.357 & 77671.12 & 1.0012 & 196.15 & 0.9924 \\
      &          &       4 & 5.387 & 77871.34 & 1.0038 & 194.04 &
      0.9818 \\
           \hline
       &           &         &       &          &        &        &        \\
       \multirow{12}{*}{5} &  \multirow{12}{*}{202}
                &       1 & 6.391 & 77600.12 & 0.9997 & 189.87 & 0.9861 \\
      &          &       1 & 6.421 & 77859.67 & 1.0030 & 188.72 & 0.9800 \\
      &          &       1 & 6.450 & 77996.08 & 1.0048 & 189.82 & 0.9858 \\
      &          &       2 & 6.582 & 78167.24 & 0.9997 & 195.86 & 1.0020 \\
      &          &       2 & 6.612 & 78393.06 & 1.0026 & 193.02 & 0.9875 \\
      &          &       2 & 6.642 & 78320.96 & 1.0017 & 189.91 & 0.9716 \\
      &          &       3 & 6.745 & 77489.71 & 0.9980 & 184.65 & 0.9970 \\
      &          &       3 & 6.774 & 77745.72 & 1.0013 & 183.84 & 0.9926 \\
      &          &       3 & 6.804 & 77746.48 & 1.0013 & 183.86 & 0.9927 \\
      &          &       4 & 6.936 & 77799.03 & 0.9993 & 181.59 & 0.9771 \\
      &          &       4 & 6.966 & 77910.98 & 1.0007 & 185.86 & 1.0001 \\
      &          &       4 & 6.996 & 78149.82 & 1.0038 & 184.81 &
     0.9944 \\
                \hline
       &           &         &       &          &        &        &        \\
       \multirow{12}{*}{6} &  \multirow{12}{*}{227}
           &       1 & 8.063 & 77432.59 & 0.9938 & 185.75 & 0.9927 \\
 &          &       1 & 8.092 & 77916.03 & 1.0000 & 182.53 & 0.9755 \\
 &          &       1 & 8.122 & 77916.40 & 1.0000 & 180.14 & 0.9627 \\
 &          &       2 & 8.254 & 77800.14 & 0.9995 & 188.38 & 0.9766 \\
 &          &       2 & 8.284 & 77805.98 & 0.9995 & 193.43 & 1.0028 \\
 &          &       2 & 8.314 & 77923.23 & 1.0011 & 194.87 & 1.0102 \\
 &          &       3 & 8.417 & 78389.06 & 0.9986 & 194.13 & 0.9965 \\
 &          &       3 & 8.446 & 78630.61 & 1.0017 & 192.12 & 0.9862 \\
 &          &       3 & 8.476 & 78515.42 & 1.0002 & 191.06 & 0.9807 \\
 &          &       4 & 8.608 & 77414.03 & 0.9979 & 198.44 & 1.0040 \\
 &          &       4 & 8.638 & 77724.12 & 1.0019 & 194.72 & 0.9852 \\
 &          &       4 & 8.668 & 77842.54 & 1.0034 & 193.93 &
     0.9812 \\
     \enddata
\end{deluxetable}




==> tab2.tex <==
\begin{deluxetable}{cccccccc}
\tabletypesize{\scriptsize}
\tablecaption{F160W Photometry Results\label{tab:F160W}}
\tablewidth{0pt}
\tablehead{
\colhead{Orbit} & \colhead{Pos. Angle} & \colhead{Dither} & \colhead{T
- JD$_{0}$} & \colhead{$\mathrm{Flux_{prim}}$} &
\colhead{$\mathrm{Flux_{prim}}$}  &\colhead{$\mathrm{Flux_{comp}}$} & \colhead{$\mathrm{Flux_{comp}}$}\\
  \colhead{}&\colhead{($^{\circ}$)}&\colhead{Position}&\colhead{[hour]}&\colhead{[$\mathrm{e^{-}/s}$]}
  &\colhead{normalized}&\colhead{[$\mathrm{e^{-}/s}$]}&\colhead{normalized}
}

\startdata
       &           &         &       &          &        &        &
       \\
              \multirow{10}{*}{1} &  \multirow{10}{*}{202}
        &       1 & 0.091 & 63247.39 & 0.9949 & 309.55 & 0.9789 \\
&        &       1 & 0.121 & 63231.17 & 0.9947 & 320.57 & 1.0138 \\
&        &       1 & 0.150 & 63234.83 & 0.9947 & 310.39 & 0.9816 \\
&        &       2 & 0.282 & 62880.74 & 0.9899 & 314.73 & 0.9965 \\
&        &       2 & 0.312 & 63170.96 & 0.9945 & 319.87 & 1.0127 \\
&        &       3 & 0.445 & 63482.02 & 0.9909 & 312.57 & 1.0003 \\
&        &       3 & 0.474 & 63876.58 & 0.9970 & 314.81 & 1.0075 \\
&        &       3 & 0.504 & 63868.25 & 0.9969 & 316.42 & 1.0126 \\
&        &       4 & 0.607 & 63268.09 & 0.9911 & 305.45 & 0.9924 \\
&        &       4 & 0.636 & 63637.60 & 0.9969 & 310.09 & 1.0074 \\
\hline
       &           &         &       &          &        &        &
       \\
              \multirow{10}{*}{2} &  \multirow{10}{*}{227}
        &       1 & 1.685 & 63800.82 & 1.0014 & 317.96 & 1.0094 \\
&        &       1 & 1.714 & 63646.56 & 0.9990 & 320.24 & 1.0167 \\
&        &       1 & 1.744 & 63712.52 & 1.0001 & 318.32 & 1.0106 \\
&        &       2 & 1.876 & 62867.13 & 0.9951 & 327.52 & 1.0173 \\
&        &       2 & 1.906 & 63215.33 & 1.0007 & 322.00 & 1.0001 \\
&        &       3 & 2.039 & 63472.43 & 0.9940 & 312.25 & 1.0059 \\
&        &       3 & 2.068 & 64211.58 & 1.0056 & 314.82 & 1.0142 \\
&        &       3 & 2.098 & 64018.46 & 1.0025 & 307.83 & 0.9917 \\
&        &       4 & 2.201 & 63356.87 & 0.9965 & 315.89 & 1.0031 \\
&        &       4 & 2.230 & 63173.89 & 0.9937 & 318.91 & 1.0127 \\
\hline
       &           &         &       &          &        &        &
       \\
              \multirow{11}{*}{3} &  \multirow{11}{*}{202}
        &       1 & 3.279 & 63508.62 & 0.9991 & 321.56 & 1.0169 \\
&        &       1 & 3.308 & 63639.15 & 1.0011 & 321.16 & 1.0156 \\
&        &       1 & 3.338 & 63817.51 & 1.0039 & 318.01 & 1.0057 \\
&        &       2 & 3.470 & 63713.27 & 1.0030 & 317.28 & 1.0046 \\
&        &       2 & 3.500 & 63948.17 & 1.0067 & 318.58 & 1.0087 \\
&        &       3 & 3.632 & 64133.71 & 1.0010 & 318.27 & 1.0185 \\
&        &       3 & 3.662 & 64148.99 & 1.0013 & 316.10 & 1.0116 \\
&        &       3 & 3.692 & 64378.74 & 1.0049 & 310.91 & 0.9950 \\
&        &       4 & 3.824 & 64067.16 & 1.0036 & 300.93 & 0.9777 \\
&        &       4 & 3.854 & 64067.97 & 1.0036 & 308.13 & 1.0011 \\
&        &       4 & 3.884 & 63910.80 & 1.0011 & 314.97 & 1.0233 \\
\hline
       &           &         &       &          &        &        &
       \\
              \multirow{11}{*}{4} &  \multirow{11}{*}{227}
        &       1 & 4.872 & 63914.07 & 1.0032 & 311.23 & 0.9880 \\
&        &       1 & 4.902 & 63884.46 & 1.0028 & 315.39 & 1.0013 \\
&        &       1 & 4.932 & 63920.45 & 1.0033 & 314.80 & 0.9994 \\
&        &       2 & 5.064 & 63364.21 & 1.0030 & 321.69 & 0.9992 \\
&        &       2 & 5.094 & 62992.57 & 0.9971 & 320.14 & 0.9944 \\
&        &       3 & 5.226 & 63789.12 & 0.9990 & 310.93 & 1.0017 \\
&        &       3 & 5.256 & 64018.91 & 1.0025 & 312.98 & 1.0083 \\
&        &       3 & 5.286 & 63849.69 & 0.9999 & 309.99 & 0.9986 \\
&        &       4 & 5.418 & 63722.64 & 1.0023 & 316.11 & 1.0038 \\
&        &       4 & 5.448 & 63707.71 & 1.0021 & 312.25 & 0.9915 \\
&        &       4 & 5.477 & 63813.00 & 1.0037 & 314.67 & 0.9992 \\
\hline
       &           &         &       &          &        &        &
       \\
              \multirow{11}{*}{5} &  \multirow{11}{*}{202}
        &       1 & 6.482 & 63771.50 & 1.0032 & 306.82 & 0.9703 \\
&        &       1 & 6.511 & 63910.88 & 1.0054 & 316.82 & 1.0019 \\
&        &       1 & 6.541 & 63759.91 & 1.0030 & 321.02 & 1.0152 \\
&        &       2 & 6.673 & 63587.56 & 1.0011 & 315.41 & 0.9986 \\
&        &       2 & 6.703 & 63817.91 & 1.0047 & 309.17 & 0.9789 \\
&        &       3 & 6.836 & 64135.94 & 1.0011 & 303.13 & 0.9701 \\
&        &       3 & 6.865 & 64302.83 & 1.0037 & 306.83 & 0.9819 \\
&        &       3 & 6.895 & 64273.25 & 1.0032 & 313.31 & 1.0027 \\
&        &       4 & 7.027 & 64005.66 & 1.0026 & 304.82 & 0.9903 \\
&        &       4 & 7.057 & 63728.45 & 0.9983 & 307.86 & 1.0002 \\
&        &       4 & 7.087 & 64020.34 & 1.0029 & 310.13 & 1.0076 \\
\hline
       &           &         &       &          &        &        &
       \\
              \multirow{11}{*}{6} &  \multirow{11}{*}{227}
        &       1 & 8.154 & 63248.40 & 0.9928 & 314.61 & 0.9988 \\
&        &       1 & 8.183 & 63573.69 & 0.9979 & 309.55 & 0.9827 \\
&        &       1 & 8.213 & 63681.11 & 0.9996 & 312.85 & 0.9932 \\
&        &       2 & 8.345 & 63367.46 & 1.0031 & 317.65 & 0.9866 \\
&        &       2 & 8.375 & 63238.70 & 1.0010 & 322.75 & 1.0025 \\
&        &       3 & 8.508 & 63746.16 & 0.9983 & 306.08 & 0.9861 \\
&        &       3 & 8.537 & 63724.29 & 0.9979 & 309.73 & 0.9978 \\
&        &       3 & 8.567 & 63874.72 & 1.0003 & 309.08 & 0.9957 \\
&        &       4 & 8.699 & 63614.87 & 1.0006 & 309.17 & 0.9817 \\
&        &       4 & 8.729 & 63530.79 & 0.9993 & 320.22 & 1.0168 \\
&        &       4 & 8.759 & 63696.84 & 1.0019 & 312.14 & 0.9912 \\
\enddata
\end{deluxetable}

